Modeling Semantic Relatedness using Global Relation Vectors

Word embedding models such as GloVe rely on co-occurrence statistics from a large corpus to learn vector representations of word meaning. These vectors have proven to capture surprisingly fine-grained semantic and syntactic information. While we may similarly expect that co-occurrence statistics can be used to capture rich information about the relationships between different words, existing approaches for modeling such relationships have mostly relied on manipulating pre-trained word vectors. In this paper, we introduce a novel method which directly learns relation vectors from co-occurrence statistics. To this end, we first introduce a variant of GloVe, in which there is an explicit connection between word vectors and PMI weighted co-occurrence vectors. We then show how relation vectors can be naturally embedded into the resulting vector space.

==> relation-classification.tex <==
%------------------------------------
\subsection{Relation Classification}

We now consider the following relation classification task: given a sentence mentioning two entities, decide which relationship is being expressed between these entities. As a standard benchmark for this task, we have used the dataset from SemEval 2010 Task 8 \cite{DBLP:conf/semeval/HendrickxKKNSPP10}. In this dataset, 9 semantic relationships are considered, in addition to a generic `other' class. Since the 9 relationships are asymmetric, we also need to determine in which direction they are expressed between the two given entities, which means that the total number of class labels is $2\times 9 + 1 = 19$. As usual, we treat this problem as a 19-class classification problem. 

Some entities in this dataset correspond to multi-word expressions. To obtain a word vector for these entities, we used the Zettair search engine to retrieve all sentences from the considered Wikipedia corpus mentioning these entities. We then computed PMI statistics for these entities by treating them as a single tokens. From these PMI statistics, we then obtain word vectors for all multi-word entities, using \eqref{eqGloVeOurVariant} but with the context word vectors fixed (similarly to how we learn the relation vectors).

Both supervised and unsupervised methods have been proposed for this task. Most supervised methods rely on a neural network architecture to learn how the embeddings of the words in the given sentence can be combined to produce a relation vector that is predictive for the considered 19 relations \cite{zeng2014relation,DBLP:conf/acl/SantosXZ15,xu2015classifying}. However, state-of-the-art results have also been obtained using the unsupervised RelEmb method, which was proposed in \cite{DBLP:conf/conll/HashimotoSMT15}, and which we will use as our main baseline. The RelEmb method relies on a form of word vector averaging, but uses word vectors from a type of embedding that was optimized specifically for this task. A crucial feature of this method is that it uses $n$-gram representations to (partially) take into account word ordering. In our experiments, we have obtained RelEmb feature vectors according to the method explained in \cite{DBLP:conf/conll/HashimotoSMT15}, and then trained a multi-class SVM classifier to make the actual prediction\footnote{Note that a softmax classifier was used instead of an SVM classifier in \cite{DBLP:conf/conll/HashimotoSMT15}; here we have used an SVM classifier for consistency with the rest of the paper.}. 

In this experiment, we will focus on $R_{ik}^2$, as it led to the best results in the previous experiments. There are several ways in which we can use this method:
\begin{itemize}
    \item Obtain triples only from the given sentence (sent).
    \item Obtain triples only from the Wikipedia corpus (corp).
    \item Obtain triples only from the Wikipedia corpus, augmented with the given sentence (sent+corp).
\end{itemize}
Note that when the Wikipedia corpus is used to learn relation vectors, our method is complementary to RelEmb. In particular, our relation vector represents the general relationship between the two entities, while the RelEmb vector encodes the specific relationship that is expressed in the given sentence. Therefore, we also consider a variant in which the RelEmb feature vector is concatenated with $R_{ik}^2$. For comparison, we also show results for the earlier baselines Diff, Conc and Avg. 

The results are shown in Table \ref{tabResultsSemEval}. \todo{discuss} \todo{omit acc from the table and explain that this is because it is not considered in the official evaluation script, which we use.}

\begin{table}
\centering
\footnotesize
\caption{Results for the relation classification task, using the SemEval 2010 Task 8 test set. \label{tabResultsSemEval}}
\begin{tabular}{|l |  cccc|}
\hline
        & Acc & Pre & Rec & F1 \\
\hline        
Diff            & 00.0 & 00.0 & 00.0 & 00.0\\ 
Conc            & 00.0 & 00.0 & 00.0 & 00.0\\ 
Avg (sent)     & 00.0 & 00.0 & 00.0 & 00.0\\  
Avg (corp)     & 00.0 & 00.0 & 00.0 & 00.0\\  
Avg (sent+corp)     & 00.0 & 00.0 & 00.0 & 00.0\\  
RelEmb      & 00.0 & 00.0 & 00.0 & 00.0\\  
$R^{2}_{ik}$ (sent) & 00.0 & 00.0 & 00.0 & 00.0\\ 
$R^{2}_{ik}$ (corp) & 00.0 & 00.0 & 00.0 & 00.0\\ 
$R^{2}_{ik}$ (sent+corp) & 00.0 & 00.0 & 00.0 & 00.0\\ 
RelEmb + $R^{2}_{ik}$ (sent) & 00.0 & 00.0 & 00.0 & 00.0\\ 
RelEmb + $R^{2}_{ik}$ (corp) & 00.0 & 00.0 & 00.0 & 00.0\\ 
RelEmb + $R^{2}_{ik}$ (sent+corp) & 00.0 & 00.0 & 00.0 & 00.0\\ 
 \hline
\end{tabular}
\end{table}

